Just ASK: Building an Architecture for Extensible Self-Service Spoken Language Understanding

This paper presents the design of the machine learning architecture that underlies the Alexa Skills Kit (ASK) a large scale Spoken Language Understanding (SLU) Software Development Kit (SDK) that enables developers to extend the capabilities of Amazon's virtual assistant, Alexa. At Amazon, the infrastructure powers over 25,000 skills deployed through the ASK, as well as AWS's Amazon Lex SLU Service. The ASK emphasizes flexibility, predictability and a rapid iteration cycle for third party developers. It imposes inductive biases that allow it to learn robust SLU models from extremely small and sparse datasets and, in doing so, removes significant barriers to entry for software developers and dialogue systems researchers.

==> alexa_ontology.tex <==

ASK promises to give developers full freedom in defining a voice experience. However, as discovered in internal beta this can lead to very poorly structured grammars. For example, we observed developers using only the concept of intents or only slot types to define entire surface area of voice interactions. This observation led to development of \textit{Alexa Meaning Representation Language (AlexaMRL)} \cite{Fan2017TransferLF}. 

\begin{comment}
Key tenets were demonstrating how to structure good grammars for VUI, re-usability of concepts across different skills, concepts should be intuitive, allow composing multiple intents and slots in single query. We leave it to the developer to pick and choose elements from AlexaMRL.
\end{comment}

AlexaMRL is composed of \textit{actions} (intents), \textit{entities} (slots), and \textit{properties}. An utterance is then defined  by a combination of actions, entity types, and properties. Similar to a programming language, the actions and entity types are classes that have properties that relate them to one another.

An intent represents an action the user wants to take. This could be searching or information, or playing a media object. The intent identifies the application which can fulfill the user request. For example, a SearchAction intent would internally refer to the API call to search engine.

An action operates on objects. An \textit{AddAction} requires an entity to be added and a target entity to be added to. This can be specified using the properties of an action. For example, AddAction has a property \textit{targetCollection} which identifies the type of list to add to and \textit{object} property which marks the type of object to be added.

An entity type grounds the objects that actions can act on or use. Entity types also have attributes, which are represented by properties. For example, \textit{LocalBusiness} is an entity type. It has properties such as business hours, address, phone number (among others). 

\begin{comment} Fig. \ref{ontofig} illustrates how an example query is represented in AlexaMRL. In this case the user wants to know present day's weather forecast for Seattle. This translates to performing a \textit{SearchAction} on \textit{WeatherForecast} object.  \textit{WeatherForecast} object is associated with properties like \textit{location} and \textit{startDate}. These properties are then grounded by their respective entity types. In this example location is grounded by \textit{City} and startDate by \textit{Date}.
\end{comment}
\begin{figure}[h]
  \centering
 \includegraphics[width=0.8\textwidth]{resources/alexa-ontology-weather.png}
 \caption{An utterance represented in AlexaMRL}
 \label{ontofig}
\end{figure}

\subsection{Exposing Query Representation to Skills }

To define a skill, a developer defines an \textit{interaction model} , which includes defining an intent schema, slot types, sample utterances, and an invocation phrase. In the intent schema instead of defining a complete semantic frame we only ask the developers to list intent and slot compatibility. Intents and slots can either be defined in a completely custom manner by skill developers, or can re-use elements of the Alexa ontology - such as actions as \textit{builtin intents} and entities as \textit{slot types}.

In order to give skill developers the benefits of the ontology, we chose to expose a useful subset enabling them to define the complete voice experience using just intents (corresponding to actions) and slot types (corresponding to entity types). Developers that choose to design their own intents with slot types, instead of using Amazon's pre-built intents, do not benefit from AlexaMRL's ability to automatically derive semantic roles from the action and entity properties. Thus, the semantic roles of the entities in an utterance must be derived from the developer provided sample utterances.

\begin{comment} We also allow the developers to take advantage of full AlexaMRL and extend it as needed in their respective skills. \end{comment}

A wide variety of utilities exist to help developers define interaction model for an Alexa Skill, including Skill Builder, a rich web interface with hints and completions and a testing console, AWS's Lex UI, which has an 'export-as-skill' option and programmatic skill management via the command-line using the Alexa Skill Management API - which also enables third party developers to start building skill development tooling.


==> devEx.tex <==

To define a skill, a developer defines an \textit{interaction model} , which consists of the intent schema, an invocation name, custom slot types and sample utterances. It establishes the skill's contract with Alexa and is used for training the spoken language understanding models for the skill. 

\subsection{Intent Schema and Custom Slot Types}\label{sec:schema}

The \textit{intent schema} specifies the intents supported by a skill and the expected slots for an intent.

An \textit{intent} is the intended action for an utterance. Developers may define their own intents or use the Amazon provided built-in intents. An intent may accept a \textit{slot} as an argument to represent an entity along with it's semantic role in the sentence. The data type of the slot is captured by the \textit{slot type}, which corresponds to entity types from the ontology.

Developers may use the Amazon provided built-in slot types or define their own \textit{custom slot types}. Each custom slot type requires a list of representative values. 
\begin{comment}
In the example below, 'Sign' is a developer-defined custom slot type and 'AMAZON.Date' is an Amazon provided built-in slot type from the Alexa Ontology.
\end{comment}
\lstdefinelanguage{json}{
        basicstyle=\ttfamily\footnotesize, 
        showstringspaces=false,
        tabsize=2,
        numbers=left,
        numberstyle=\tiny\color{codegray},
        caption={Sample Intent Schema for a Horoscope skill from the ASK Documentation},
        breaklines=true
}

\begin{comment}
\begin{lstlisting}[language=json,firstnumber=1]
{
  "intents": [
    {
      "intent": "GetHoroscope",
      "slots": [
        {
          "name": "Sign",
          "type": "ZODIAC_SIGNS"
        },
        {
          "name": "Date",
          "type": "AMAZON.DATE"
        }
      ]
    }
  ]
}
\end{lstlisting}
\end{comment}

\textit{Sample utterances} form the training data used for building spoken language understanding models. Each sample is labelled with an intent followed by an utterance corresponding to the intent. 

\begin{comment}
\lstdefinelanguage{utterance_format}{
        basicstyle=\ttfamily\footnotesize, 
        showstringspaces=false,
        numbers=left,
        numberstyle=\tiny\color{codegray},
        caption={Sample Utterances for a Horoscope skill},
        breaklines=true
}
\begin{lstlisting}[language=utterance_format,firstnumber=1]
GetHoroscope what is the horoscope for {Sign}
GetHoroscope what will the horoscope for {Sign} be on {Date}
GetHoroscope get me my horoscope
GetHoroscope {Sign}
\end{lstlisting}
\end{comment}

Thus a set of sample utterances in conjuction with the developer provided custom types and the Alexa Ontology defines a grammar. 
The utterances within the grammar are guaranteed to be supported deterministically.
This simplifies  skill design and testing for developers,  however because of a high degree of variance present in spoken language speech, 
this grammar is insufficient to serve customers in a real world use case, 
which motivates the need to train statistical models that are better suited to noisy input from an real world speech and an underlying ASR system.

The wide variety of utilities exist to help developers define interaction model for an Alexa Skill, including Skill Builder, 
a rich web interface with hints and completions and a testing console, AWS's Lex UI, which has an 'export-as-skill' option and programmatic skill
management via the command-line using the Alexa Skill Management API - which also enables third party developers
to start building skill development tooling.


==> nlu_data_prep.tex <==
A skill developer provides example utterances for the skill using a simple grammar. We infer a grammar from the sample utterances and intent schema provided by the developer, this is encoded efficiently as a wFST. This representation is useful because we can impose arbitrary distributional priors on on the grammar. We infer a distribution over intents and slots from the sample utterances. As the data in sample utterances is often imbalanced we impose a uniform prior on the grammar ingested from such data. However, we keep this as a configurable switch which is turned off when the training data is ingested from the usage pattern of the skill.  

The distributionally weighted FST representation can be used directly with common text processing models designed to work with text such as CRFs \cite{lafferty2001conditional} and LSTMs \cite{lample2016neural} by sampling utterances according to the distributional priors and feeding them into the respective models as training data via a data recombination technique similar to \cite{jia2016data}. Another way to utilize the grammar is to train directly on the lattice itself \cite{ladhak2016latticernn}.

